Constant Random Perturbations Provide Adversarial Robustness with Minimal Effect on Accuracy

This paper proposes an attack-independent (non-adversarial training) technique for improving adversarial robustness of neural network models, with minimal loss of standard accuracy. We suggest creating a neighborhood around each training example, such that the label is kept constant for all inputs within that neighborhood. Unlike previous work that follows a similar principle, we apply this idea by extending the training set with multiple perturbations for each training example, drawn from within the neighborhood. These perturbations are model independent, and remain constant throughout the entire training process. We analyzed our method empirically on MNIST, SVHN, and CIFAR-10, under different attacks and conditions. Results suggest that the proposed approach improves standard accuracy over other defenses while having increased robustness compared to vanilla adversarial training.

==> CRP Provide Adversarial Robustness with Minimal Effect on Accuracy WORKSHOP ICLR 2021 m/experiments.tex <==
\section{Experimental Results}
\label{sec: experiments}


This section presents our empirical evaluation of the proposed method on the CIFAR-10 dataset under different settings (results for MNIST and SVHN are in the Appendix). Our approach is based on constant perturbations that are sampled once at the beginning of the training phase; hence we need to consider the randomness in selecting a good or bad set of perturbations. Therefore, we performed every experiment five times and reported the average accuracy and standard deviation of these experiments, alongside the best model among the five. The perturbations were sampled from a uniform distribution $\mathcal{U}(-16/255,16/255)$. 

We start by presenting our robustness under both white-box and black-box attacks in \tableref{tab:table_cifar10_gen}. We used $\epsilon = 8/255$. The PGD attack was used with a step size  $\eta = 2/255$. We denote by PGD$^n$ the attack created with $n$ iterations. For the black-box setup, we trained 5 models with our method and attacked each one of them with adversarial examples generated from the other 4 models.


\begin{table}[h!]
\vspace{-0.25cm}
\begin{center}
\caption{\it Accuracy of the model trained and tested on CIFAR-10 under different attacks with $\epsilon = 8/255$. \topmodel $~$ represents the accuracy of the best model out of 5.}
\label{tab:table_cifar10_gen}
\footnotesize
\begin{tabular}{lcccc} 

\hline
\hline
\multirow{2}{*}{Setting} & \multicolumn{2}{c}{White-box attack [\%]} & \multicolumn{2}{c}{Black-box attack [\%]} \\
  & Accuracy[\%] & \topmodel [\%]  & Accuracy[\%] & \topmodel [\%] \\
\hline
\hline
No Attack  & $91.56 \pm 0.51$ &  $92.07$ & $91.56 \pm 0.51$ &  $92.07$\\
\hline
FGSM  & $64.09 \pm 2.66$&  $66.75$   & $69.17 \pm 0.58$ &  $69.75$\\
PGD$^{7}$ & $52.22 \pm 4.83$ & $58.93$ & $67.74 \pm 1.63$ &  $69.37$ \\
% PGD$^{10}$ & $50.15 \pm 5.94$&  $56.09$ & -- & --  \\
PGD$^{20}$  & $46.41 \pm 8.00$&  $55.51$ & $66.45 \pm 1.76$&  $68.21$\\
% PGD$^{40}$   & $43.25 \pm 9.96$&  $53.21$ & -- & --\\
PGD$^{100}$  & $40.76 \pm 11.16$&  $51.92$ & $65.23 \pm 2.20$ &  $67.43$ \\
\hline
\hline
\end{tabular}
\end{center}
\vspace{-0.4cm}

\end{table}


We can observe from the small standard deviation that the standard accuracy of the models is comparable. Similarly, robustness against a weaker adversary such as FGSM, is also similar between models, which is evident from the low variance. Against a stronger adversary such as PGD the gap increases as the number of iterations increases. Nevertheless, if we look at our best model, its robustness is higher than some other models. This indicates the importance of selecting a good sample of the perturbations. 

Additionally, our method's transferability is consistent between the different models, as can be observed from the standard deviation, which is lower for black-box attacks than white-box attack. It is clear that the proposed method adds robustness against the transferability of adversarial examples from other models, in addition to the increased robustness of white-box attacks.

\begin{table}[t!]
\vspace{-0.25cm}
\centering
\caption{\it Comparing results on SVHN of our method with two models of ME-NET
\citep{yang2019me} with different classification accuracy and with \citet{madry2018towards} as reported in \citep{yang2019me}. Attacks are \textbf{white-box} attacks with $\epsilon = 8/255$.}
\label{tab:table_svhn_comp}
\footnotesize
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lccc} 
\hline
\hline%\\[-.3cm]
% FGSM 72.67
Method & No attack & PGD$^{20}$ & PGD$^{100}$\\
\hline
% Proposed 15 perturb.  & 94.29 & 69.79 & 69.78\\
Proposed $\mathcal{U}(-8/255,8/255)$\!\!\!  & 94.13 &
74.30 & 74.23\\
Proposed $\mathcal{U}(-16/255,16/255)$ 20 pert.\!\!\!  & \textbf{94.28} &
\textbf{80.32} & \textbf{80.21}\\
%Proposed $\mathcal{U}(-8/255,8/255)$\!\!\!  & \textbf{95.05} & 60.13 & $60.04$\\%extra dropout
Proposed $\mathcal{U}(-16/255,16/255)$\!\!\!  & 93.73 & 69.62 & 69.61\\
\citet{madry2018towards} & 87.40 & 48.40 & 47.50 \\
ME-NET (0.2--0.4) & 87.60 & 75.8 & 69.80\\
ME-NET (0.8--1.0) & 93.50 & 41.40 & 35.50\\
\hline
\hline
\vspace{-0.7cm}
\end{tabular}
\end{table}

%\subsection{Comparison to other methods}
We now turn to compare our approach to state-of-the-art methods, which use adversarial training. We start with the SVHN dataset. In \tableref{tab:table_svhn_comp} we state the result of three of our models: our best model trained with $\mathcal{U}(-16/255,16/255)$ with ten and twenty perturbations and with $\mathcal{U}(-8/255,8/255)$\footnote{Additional results on SVHN with different distribution bound are given in Appendix.}. These are compared with \citet{madry2018towards} and ME-NET \citep{yang2019me}\footnote{The results of \citet{madry2018towards} on SVHN are taken from \citet{yang2019me}.}.   We show the performance of two different models of ME-NET, one more robust and one with higher classification accuracy. We can see that our model trained with 20 perturbations has the highest accuracy and robustness. Moreover, in terms of standard accuracy, all of our models have higher accuracy in both settings. In terms of robustness, while for PGD with 20 iterations, our models trained with ten perturbations have lower adversarial accuracy than ME-NET, for PGD with 100 iterations, our model trained with $\mathcal{U}(-8/255,8/255)$ has higher robustness than ME-NET. Furthermore, our model has higher robustness and higher classification accuracy than the ME-NET model with the highest classification accuracy.


\begin{table}[h!]
\begin{center}
\vspace{-0.3cm}
\caption{\it Comparing our method to other methods based on adversarial training on CIFAR-10 using $\epsilon = 8/255$. For PGD we used step size of $2/255$ with 20 iterations Proposed method$^{\text{best}}$ represents the best model out of the five we trained.}
\label{tab:madri_cifar_compcifar}
\footnotesize
\begin{tabular}{lcccc} 
\hline\hline
Method & No Attack & FGSM & PGD$^{20}$ & PGD$^{100}$\\
\hline\hline
Proposed Method$^{\text{best}}$ & \textbf{91.77} & 66.75 & $55.51$ & 51.92\\
 \cite{madry2018towards} & $87.30$ & $56.1$ & $45.80$ & $45.05$\\
 RST$_{adv}$ {\citep{carmon2019unlabeled}} & $89.7 \pm0.1$ & 69.68 & \textbf{63.10} & \textbf{62.14}\\
 TRADES {\citep{zhang2019theoretically}} & $84.92$ & $60.87$ & $55.38$ & 55.13\\
 ME-NET {\citep{yang2019me}} $p: 0.4 \rightarrow 0.6$&  85.50 & \textbf{71.39} & 61.60 & 55.90 \\
  ME-NET {\citep{yang2019me}} $p: 0.6 \rightarrow 0.8$ &  91.00 & - & 58.00 & 53.40 \\
\hline\hline
\end{tabular}
\end{center}
\vspace{-0.4cm}
\end{table}



Next, we turn to compare our performance on CIFAR-10. Results are shown in \tableref{tab:madri_cifar_compcifar}. When comparing our method to other defenses, we should consider that they incorporated additional use of data or computations. Specifically, RST$_{adv}$ \citep{carmon2019unlabeled} used 500k additional unlabeled examples compared to other methods reported. ME-NET \citep{yang2019me} performs matrix estimation on top of adversarial training within the network's pipeline, for every PGD iteration. Additionally, we would like to stress that our method does not incorporate an attack within any step of our training. \begin{wrapfigure}{r}{0.43\textwidth}
\vspace{-0.2cm}
\centering
 \includegraphics[width=0.9\linewidth]{figures/robustacrossepssns.png}
    % \caption{}
    %  CIFAR-10: Robustness of our different methods, across different values of $ \epsilon$.}
    %  \label{fig:rob}
% \hspace{-0.3cm}
\vspace{-0.3cm}
\caption{\footnotesize{CIFAR 10: Robustness of our different methods, across different values of $ \epsilon$.}}
\vspace{-0.6cm}
\label{fig:figures}
\end{wrapfigure}We can observe in \tableref{tab:madri_cifar_compcifar} that the classification accuracy (``no attack'') is high, while the robustness of our model is favorably compared to \citet{madry2018towards}, consistently.  


Finally, we tested how our model's robustness hold across different values of epsilon against PGD with 20 iterations, and compared it to the robustness of other methods. Results are shown in Fig. 1. It can be observed that for our models, up to $\epsilon = 5$ there is a linear decay in robustness accuracy, and then the decay is more subtle. On the other hand, for models based on adversarial training, the decay remains approximately linear. 
% Finally, we show the effect of the number of perturbations on adversarial accuracy. We trained models with one, five, and ten (five of each) perturbations. Results of average adversarial accuracy are shown in Appendix Fig. 1 (right). We can observe that using more perturbations increases robustness. It seems that using even 10 perturbations per example did not reach the full potential of the possible robustness, and further research needs to be done to understand how to sample effectively with more perturbations.





 % \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{.45\linewidth}
%   \centering
%  \includegraphics[width=0.7\linewidth]{figures/robustacrossepssns.png}
%     % \caption{}
%     %  CIFAR-10: Robustness of our different methods, across different values of $ \epsilon$.}
%      \label{fig:rob}
% \end{subfigure}%
% \hspace{0.3cm}
% \begin{subfigure}[t]{.45\linewidth}
%   \centering
%   \includegraphics[width=0.7\linewidth]{figures/pertcountsns.png}
%   %\caption{}
% %   CIFAR-10: Effect of the number of perturbations on average adversarial accuracy of five models.}
% %   
% \label{fig:perteffect}
% \end{subfigure}
% \caption{CIFAR 10: Robustness of our different methods, across different values of $ \epsilon$ (left). Effect of the number of perturbations on average adversarial accuracy of five models (right).}
% \vspace{-0.6cm}
% \label{fig:figures}
% \end{figure}


==> CRP Provide Adversarial Robustness with Minimal Effect on Accuracy WORKSHOP ICLR 2021 m/introduction.tex <==
\section{Introduction}
\label{intro_ewn}
Deep neural networks are susceptible to {\em adversarial attacks} -- the presentation of almost imperceptibly manipulated ``adversarial'' inputs that cause the system to misclassify them \citep{goodfellow2014explaining, moosavi2016deepfool, kurakin2016adversarial,apernot2017practical,fawzi2018analysis, gilmer2019adversarial, papernot2016distillation, cisse2017parseval}.
%This concerning phenomenon, which attests to the fragility of machine learning in general, and of deep learning in particular \citep{apernot2017practical}, has triggered an active line of research aimed at understanding it \citep{fawzi2018analysis, gilmer2019adversarial}, and increasing the robustness of neural networks to such attacks \citep{papernot2016distillation, cisse2017parseval}.  
%
A variety of defense techniques have been proposed in the literature to address this problem. The most successful line of work is {\em adversarial training} \citep{szegedy2013properties, goodfellow2014explaining,  madry2018towards, zhang2019theoretically, carmon2019unlabeled}, which attempts to enhance the robustness of the network by including adversarial examples in the training data itself, with the implicit purpose of ``teaching'' the network not to be fooled by such data instances. Extensions attempt to further improve the robustness through the additional use of pre-processing techniques, on top of the adversarial training \citep{xie2019feature, yang2019me, hendrycks2019using}.

Conventional training views each training example as a \emph{zero volume} element in the space where the output must be correctly predicted. While the continuity of the various activation functions in the network implicitly creates neighborhoods around each training example, such that if a given input falls within this neighborhood, it will be classified correctly \citep{xu2012robustnessvi}, this is not explicitly enforced. Moreover, this neighborhood, might be too small to be robust against adversarial examples. 

% \todo{stress they incorporate PGD}
Adversarial training explicitly expands the neighborhood around each training example in adversarially sensitive directions. Practically, this is done by selecting an \emph{approximation} of the worst-case adversary: each training example is replaced with an adversarial one that lies within an $\epsilon$ neighborhood of the original input, under some $\ell_p$ norm. Since the adversarially-sensitive directions depend on the model parameters which are continually updated during training, the adversarially modified training instances themselves must be recomputed in each epoch of training. 
This approach achieves increased robustness, often at the cost of standard classification accuracy on non-adversarial data, which becomes more prominent as the input dimension grows \citep{zhang2019theoretically, tsipras2018robustness, carmon2019unlabeled}.

In this paper, we take a different approach and consider each training instance to represent a ball in the input space centered at that instance, such that the label for the instance holds within the entire ball. The ball itself is fixed for each instance, and is not dependent on the model, which is trained to minimize the expected loss over the ball. We approximate this expectation over the ball, by sampling several points within it. This gives us \emph{constant random perturbations} -- a set of perturbations are sampled a priori for every training example from a chosen distribution of an $\epsilon$-bounded domain. We extend the training set with these perturbed examples and keep them constant throughout the training process.

It must be noted that this method differs from conventional adversarial training in two ways: first, unlike adversarial training, the perturbations added to the training set depend only the training instance and do not depend on the model or the adversary. Secondly, also unlike adversarial training where adversarial perturbations must be updated in each iteration of training, the perturbed samples we draw are drawn once and kept fixed during training.

We analyzed the proposed method empirically, under different conditions and under various attacks. We evaluate the standard classification accuracy and adversarial accuracy on MNIST, SVHN, and CIFAR-10. Our method depends on the specific set of perturbed samples added to the training set, and its performance may vary with the specific set of samples drawn. To account for this, for each experiment, we sampled five different perturbation sets and trained a different model. Each result is reported using the average and the standard deviation over the set of models. We also report the result of the best model. We show empirically that using constant perturbation increases robustness compared to standard training while having higher baseline classification accuracy than adversarial training. While practically we could sample only ten perturbations per training example, we show that the robustness could have been further improved using more perturbations. 

%[topsep=-1pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,leftmargin=10pt]
Our contribution:
\begin{itemize}[leftmargin=*, topsep=-1pt,noitemsep]
  \item Our approach is attack independent. Compared to previous work, we do not incorporate any adversarial attacks as a part of the training.
  \item Our method is easy to implement. We augment the training set once by adding additional perturbed examples. Other methods  pre-process or manipulate the training data every epoch. Nonetheless, our method is computationally equivalent to the vanilla adversarial training, since the generation of a PGD attack for every example at each iteration is computationally the same as adding one perturbed input to the training set.
  \item Our method has higher classification accuracy than other defenses alongside a higher robustness compared to standard models, and \citet{madry2018towards}. We alleviate robustness by over $50\%$ consistently throughout several datasets: MNIST, SVHN, and CIFAR-10.
\end{itemize}

The implementation of the method is available online\footnote{\url{https://anonymous.4open.science/r/0eb2084e-04ca-488d-92da-05076729a2de/}}.


==> CRP Provide Adversarial Robustness with Minimal Effect on Accuracy WORKSHOP ICLR 2021 m/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
% \def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
% \def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> CRP Provide Adversarial Robustness with Minimal Effect on Accuracy WORKSHOP ICLR 2021 m/problem_setting.tex <==
%!TEX root = main.tex

\section{Problem Setting}\label{sec:problem_setting}

We denote $\X \subseteq \mathbb{R}^d$ as the set of our input examples, which are represented as $d$-dimensional vectors, and we denote $\Y = \{1,...,M\}$ as the set of class labels. Let $\f: \X \to \Y$ be a neural network with parameters $\theta$, that takes an input from $\X$ and predicts its associated label in $\Y$. During training the parameters $\theta$ are estimated by minimizing the surrogate loss function $\ell(x, y;\theta)$, where $x\in\X$ and $y\in\Y$, over a training set of $M$ examples, $\mathcal{S}=\{(x_i, y_i),~ i = 1\cdots M\}$, as follows:
\begin{equation}
\label{eq:tstar}
\theta^* = \argmin_{\theta}  \sum_{(x,y) \in \mathcal{S}}  \ell(x, y; \theta),
\end{equation}
where $\theta^*$ is the estimated parameters. 

% Given an input $x$ with a label $y$, and a trained network $\f$ with a \emph{fixed} set of parameters $\theta$,  adversarial example $\tdxa=x+\delta$ is generated by finding the perturbation $\delta$ that maximizes the loss as follows:
% \begin{equation}\label{eq:adversarial_optim}
% \delta = \argmax_{\|\delta\|_p \le \epsilon} \ell(x + \delta, y; \theta^*),
% \end{equation}
% where $\epsilon$ represents the strength of the adversary measured using the $p$-norm. One possible solution to this optimization problem is done by taking the first order Taylor expansion with $p=\infty$. This is called  the \textit{fast gradient sign method} (FGSM) and was proposed by \cite{goodfellow2014explaining}:
% \begin{equation}\label{eq:fgsm}
% \tdxa^\mathrm{FGSM} = x + \epsilon \, \sign(\nabla_x \, \ell(x + \delta, y; \theta^*) ).
% \end{equation}

Our goal is to represent each training example by a ball in which the label is kept constant. 
%The parameters of the model should be learned so as that the label is the same for the entire ball. 
Let $B^{\infty}_{\epsilon}(x)=\{z\in\X : \|z - x \|_\infty \le \epsilon \}$ be the $\ell_\infty$ ball of radius $\epsilon$ around $x$. We define the {\em ball} loss function $\bar{\ell}(x,y;\theta)$ as
\begin{equation}
    \bar{\ell}(x,y;\theta) = \int_{B^{\infty}_\epsilon(0)} \ell(x+\delta,y;\theta) \, d q_\epsilon(\delta)~,
    \label{eq:loss1}
\end{equation}
where $\ell(x,y;\theta)$ is the (point) loss computed at $x$, and $q_\epsilon(\delta)$ is a probability distribution function of the random variable $\delta$. The above Lebesgue integral is generally infeasible to compute; however when $q_\epsilon(\delta)$ is the probability of $\delta$, \eqref{eq:loss1} becomes an expectation of the loss over the ball, {\em i.e.}, $
\bar{\ell}(x,y;\theta) = \mathbb{E}_{\delta\sim q_{\epsilon}} \Big[  \ell(x+\delta,y;\theta) \Big].
$
%The estimates for the optimal network parameters $\theta^*$ are obtained as
%\begin{equation}
%\theta^* = \argmin_\theta \sum_{(x,y) \in \mathcal{S}} \mathbb{E}_{\delta\sim q_{\epsilon}} \Big[  \ell(x+\delta,y;\theta) \Big].
%\end{equation}

Since this expectation is infeasible to compute explicitly, we replace it with an empirical average, by drawing $K$ samples from ball around it, according to the distribution $q_\epsilon(\delta)$. Formally, for the training example $(x, y)$, we add a set of perturbed examples $(x+\delta_j, y)$, where $j\in\{1,\ldots,K\}$, $\delta_i \sim q_\epsilon$, and $q_\epsilon$ is a probability distribution function of random variables bounded by $\epsilon$. The network parameters are found by minimizing the average loss as follows:
\begin{equation}
\theta^* = \argmin_\theta \sum_{(x,y) \in \mathcal{S}} \sum_{j=1}^K  \ell(x+\delta_j,y;\theta),
\label{eq:opt1}
\end{equation}
where $\delta \sim q_{\epsilon}$, and $\delta\in[-\epsilon,\epsilon]^d$. 

The samples $(x+\delta_j, y),~j=1\cdots K$ are drawn only once for each training instance, at the outset. This is in contrast to other methods \citep[e.g.,][]{pmlr-v97-cohen19c}, which perturb the inputs at every epoch. We will refer to our approach as \emph{constant perturbations} and the latter sampling techniques as \emph{variable perturbations}. In practice, we aggregate all generated training samples into a single set $\bar{\mathcal{S}}$ of size $KM$, and simply redefine the optimization as
\begin{equation}
\theta^* = \argmin_\theta \sum_{(x,y) \in \bar{\mathcal{S}}}  \ell(x,y;\theta),
\label{eq:opt2}
\end{equation}
Subsequent optimization treats the $KM$ instances in the augmented set as independent training samples, and further training proceeds as usual.

==> CRP Provide Adversarial Robustness with Minimal Effect on Accuracy WORKSHOP ICLR 2021 m/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
Previous works explored the use of random perturbations (sampled anew at every epoch) to increase robustness. They can be used during training \citep{szegedy2013properties, goodfellow2014explaining, pmlr-v97-cohen19c, lecuyer2019certified, zhu2019freelb} or during inference \citep{pmlr-v97-cohen19c, salman2019provably, zhang2019defending}.
The use of random perturbation alone was not effective enough to defend against an adversary. 

The idea that additional data can improve robustness, was shown theoretically and empirically \citep{schmidt2018adversarially} even for unlabeled data \citep{hendrycks2019using, carmon2019unlabeled, alayrac2019labels, zhai2019adversarially}. Our work supports this idea by adding perturbed or augmented variations of the original training examples to the training set.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}
Previous works explored the use of random perturbations (sampled anew at every epoch) to increase robustness. They can be used during training \citep{szegedy2013properties, goodfellow2014explaining, pmlr-v97-cohen19c, lecuyer2019certified, zhu2019freelb} or during inference \citep{pmlr-v97-cohen19c, salman2019provably, zhang2019defending}.
The use of random perturbation alone was not effective enough to defend against an adversary. 

The idea that additional data can improve robustness, was shown theoretically and empirically \citep{schmidt2018adversarially} even for unlabeled data \citep{hendrycks2019using, carmon2019unlabeled, alayrac2019labels, zhai2019adversarially}. Our work supports this idea by adding perturbed or augmented variations of the original training examples to the training set.
